Saddle-to-Saddle Dynamics in Diagonal Linear Networks

In this paper we fully describe the trajectory of gradient flow over diagonal linear networks in the limit of vanishing initialisation. We show that the limiting flow successively jumps from a saddle of the training loss to another until reaching the minimum $\ell_1$-norm solution. This saddle-to-saddle dynamics translates to an incremental learning process as each saddle corresponds to the minimiser of the loss constrained to an active set outside of which the coordinates must be zero. We explicitly characterise the visited saddles as well as the jumping times through a recursive algorithm reminiscent of the LARS algorithm used for computing the Lasso path. Our proof leverages a convenient arc-length time-reparametrisation which enables to keep track of the heteroclinic transitions between the jumps. Our analysis requires negligible assumptions on the data, applies to both under and overparametrised settings and covers complex cases where there is no monotonicity of the number of active coordinates. We provide numerical experiments to support our findings.

==> Sections/left_overs.tex <==
% \small


% \Snote{where to put this paragraph?}
% however we recall the two classical settings which are covered by our results.
% The \textit{underparametrised} setting, where $d\leq n$ and for which there exists a unique solution $\beta^\star = \argmin_\beta L(\beta)$.
% %
% The \textit{overparametrised} setting, where $d > n$ and where there exists an infinite number of minimisers $\beta^\star \in \R^d$ which attain zero training loss and which correspond to linear predictors that perfectly fit the training data, \textit{i.e.} $y_i = \langle \beta^\star, x_i \rangle$ for all $1 \leq i \leq n$. These predictors are referred to as   \textit{interpolators}. %The only assumption we need on the inputs

% \Snote{Also this}

% \myparagraph{Taking the initialisation scale to $0$, mirror point of view.} 
% %
% As mentioned before, the iterates $\tbeta^\alpha_t$ stay stuck at $\mathbf{0}$ when $\alpha \to 0$. The mirror flow point of view sheds a new light on this observation.
% %
% Differentiating the left side of equation \ref{eq:ode_betaa} and computing the Hessian of $\phi_\alpha$,  the iterates $\tbeta^\alpha_t$ are shown to follow $\dot{\tbeta}^\alpha_t = - \sqrt{  (\tbeta^\alpha_t)^2 + \alpha^4} \odot \nabla L(\tbeta^\alpha_t)$.
% %
% Taking $\alpha \to 0$, this flow is informally equivalent to $\dot{\tbeta}_t = - |\tbeta_t| \odot \nabla L(\tbeta_t)$ for which $\mathbf{0}$ is a fixed point as well as all vectors $\beta_c = \beta_{w_c}$ where $w_c$ is a saddle point of $F$ (following \Cref{prop:function_F}).

% \Snote{this}


% \myparagraph{Notations and terminology.} In all generality we denote by $\beta^\star_{\ell_1} \coloneqq  \argmin_{\beta^\star \in \argmin_\beta L(\beta)} \Vert \beta^\star \Vert_1$ the minimum $\ell_1$-norm solution, we point out that it simplifies to $\beta^\star_{\ell_1}  \coloneqq \argmin_{\beta} L(\beta)$ in the underparametrised setting, and to $\beta^\star_{\ell_1} \coloneqq \argmin_{y_i = \langle x_i, \beta^\star \rangle, \forall i} \Vert \beta^\star \Vert_1$ in the overparametrised setting. For an integer $d$, we denote $[d]$ the set $\{1, \dots, d \}$ and for $i \in [d]$ we denote $\{ i \}^C$ the complementary set of $\{i\}$ in $[d]$. We abuse of the terminology of ``saddle'' when speaking of a point $\beta_c \in \R^d$ which \textbf{is not} an actual saddle of the loss $L$ which is convex. We use it because it corresponds to a point $w_c \in \R^{2d}$ which is a saddle of the non-convex loss $F$.

% \begin{prop}\label{prop:behaviour_nablaphia}
% Let $(\tilde{\beta}^{\alpha})_{\alpha > 0}$ such that $(\tilde{\beta}^\alpha, \nabla \ttphi_\alpha(\ttbeta^\alpha)) \underset{\alpha \to 0}{\longrightarrow} (\ttbeta, \tilde{\eta}) \in \R^d \times \R^d$, then it holds that:
% \[\tilde{\eta} \in \partial \Vert \tilde{\beta} \Vert_1 \qquad \mathrm{where} \qquad \sg{\tilde{\beta}} = \large
% \substack{  
% \ \ \{1\}  \  \  \ \   \mathrm{if} \ \ \   \tilde{\beta} > 0 \\
% \ \{-1\}  \  \ \    \mathrm{if} \ \ \   \tilde{\beta} < 0 \\
% [-1, 1] \  \ \   \mathrm{if} \ \ \   \tilde{\beta} = 0 } \ \ .\]
% % where we write subdifferential of the $\ell_1$-norm as 
% %  $\sg{\tilde{\beta}} = \{1\}$ if $   \tilde{\beta} > 0 ,
% %  \ \{-1\}$ if $\tilde{\beta} < 0$ and $[-1, 1]$ if $ \tilde{\beta} = 0 $.
% \end{prop}


% \textbf{Jump at time $t_1$.} We show that there must be a discontinuous jump at time $t_1$.
% %
% To understand this claim, we consider $\tilde{\beta}^\alpha_t$ for very small $\alpha$. Differentiating the left side from \Cref{eq:process_integral_form} and computing the Hessian of $\ttphi_\al$, we obtain that $\dd \tilde{\beta}^\alpha_t = - \ln(1 / \alpha) \sqrt{(\tilde{\beta}^\alpha_t)^2 + \alpha^4} \odot \nabla L(\tilde{\beta}^\alpha_t) \sim - \ln(1 / \alpha) \vert \tilde{\beta}^\alpha_t \vert \odot  \nabla L(\tilde{\beta}^\alpha_t) \  (*)$. 
% %
% Since $t_1$ corresponds to the time the iterates leave the first saddle,  $\tilde{\beta}^\alpha_{t_1}$ cannot converge to a fixed point of $\dot{\beta}_t = - \vert \beta_t \vert \odot \nabla L(\beta_t)$.
% %
% Therefore $(*)$ entails $\Vert \dot{\tilde{\beta}}^\alpha_t \Vert \to + \infty$ as $\alpha \to 0$, which translates into a jump. 
% %
% Following the jump, the velocity should  return to a bounded state and $(*)$ implies that the iterates can only stick to another saddle where $\vert \beta \vert \odot \nabla L(\beta) = \mathbf{0}$.




% The procedure for identifying and characterising these saddles as well as the jump times is given by a standalone algorithm outlined in Algorithm~\ref{alg:algo}. We first verify that all the steps are well defined and that the algorithm terminates in a finite number of iterations in the following proposition.  The proof is deferred to \Cref{app:sec:proofprop2}.
% %



% \begin{restatable}{prop}{lemmaalg}\label{lemma:alg_defined}
% Algorithm~\ref{alg:algo} is well defined: at each iteration (i) the attribution of $\Delta$ is well defined as $\Delta < + \infty$, (ii) the constrained minimisation problem has a unique solution and the attribution of the value of $\beta$ is therefore well-founded. Furthermore, along the loops: the iterates $\beta$ have at most $n$ non-zero coordinates, the loss is strictly decreasing and the algorithm terminates in at most $\min \big (2^d, \sum_{k=0}^{n} {d \choose k} \big )$ steps by outputting the minimum $\ell_1$-norm solution $\beta^\star_{\ell_1}$.
% \end{restatable}
%  \Cref{lemma:alg_defined}  highlights that Algorithm~\ref{alg:algo} is on its own an algorithm of interest for finding the minimum $\ell_1$-norm solution in an overparametrised regression setting. We point out that the provided upperbound on the number of iterations is very crude and could certainly be improved. However, analysing Algorithm \ref{alg:algo} is not the focus of our paper.
% %\vspace{0.3em}




% The idea is similar to the Homotopy algorithm which is used to find the Lasso path: we start from $\mathbf{0}$ and successively look at the breaking times of \Cref{eq:limit_process} and determine the unique update of $\tilde{\beta}_t$ that keeps the conditions satisfied.  Let us denote $s_t \coloneqq - \int_0^t \nabla L(\tilde{\beta}^\circ_s) \dd s$.  

% \textbf{Original saddle: the iterates are stuck at $\mathbf{0}$.} 
% %
%  Intuitively one can think of the proof as a "continuous recursion" as follows: $\beta_t = \mathbf{0}$ on $[0, t)$ implies, by its definition, that $s_t = - t \cdot \nabla L(\beta_0)$. Now from (\ref{prop3})  $s_t \in (-1, 1)$ implies $\beta_t = \mathbf{0}$ . This "recursion" holds until a coordinate of $- t \cdot \nabla L(\beta_0)$ hits $\pm 1$, i.e, until the time $t_{\mathrm{break}} = \inf \{ t \geq 0, \exists i \in [d], -t \cdot \nabla L(\beta_0) = \pm 1 \} = 1 / \Vert \nabla L(\beta_0) \Vert_\infty $. 
% %
%  Let $i_{\mathrm{break}}$ be the coordinate which reaches $\pm 1$ at time $t_{\mathrm{break}}$. For simplicity assume that it is unique, and w.l.o.g. assume that $s_t(i_{\mathrm{break}}) = +1$.

% \textbf{The iterates must jump.} At time $t_{\mathrm{break}}$, we now show that: (i) the coordinate $i_{\mathrm{break}}$ must jump, (ii) the others must stay at $0$. Consider an interval $t \in (t_{\mathrm{break}}, t_{\mathrm{break}} + \varepsilon)$. Indeed by (\ref{prop1}), $s_t(\{ i_{\mathrm{break}} \}^C ) \in (-1, 1)$, and hence $\ttbeta^\circ_t( \{ i_{\mathrm{break}} \}^C ) = \mathrm{0}$ from (\ref{prop3}). Now assume that $\beta_t(i_{\mathrm{break}})$ is still equal to $0$ for $t \in (t_{\mathrm{break}}, t_{\mathrm{break}} + \varepsilon)$, then $s_t$ would still be equal to $-t \cdot \nabla L(\beta_0 = \mathbf{0})$ and $s_t(i_{\mathrm{break}}) > 1$ which contradicts contradicting (\ref{prop2}). Therefore the first jump time is $t_{\mathrm{break}}$:   $t_1 = t_{\mathrm{break}}$.

% \textbf{Saddle $\beta_1$?} The question is now to determine, where the iterates have jumped: i.e., what is the value of $\beta_1$ for $t \in (t_1, t_2)$? As shown in the previous paragraph: $\ttbeta^\circ_t(\{ i_{\mathrm{break}} \}^C) = \beta_1(\{ i_{\mathrm{break}} \}^C )= \mathbf{0}$ and $\beta_1( i_{\mathrm{break}}  ) \neq 0$. Recall that w.l.o.g we assumed that $s_{t_1}(i_{\mathrm{break}}) = +1$, therefore from \ref{prop4}, $\beta_1( i_{\mathrm{break}}  ) > 0$ and from \ref{prop5}, $s_t(i_{\mathrm{break}}) = 1$ for $t \in (t_1, t_2)$. On the other hand, from the definition of $s_t$ we can also write, $s_t(\ib) = +1 - (t-t_1) [\nabla L(\beta_1)]_\ib $ which leads to $[\nabla L(\beta_1)]_\ib = 0$. Notice that the two conditions $\beta_1(\{ i_{\mathrm{break}} \}^C )= \mathbf{0}$ and $[\nabla L(\beta_1)]_\ib = 0$ uniquely determines $\beta_1$ as being the unique solution of 
% \begin{align}
%     \beta_1 = \argmin_{\substack{\beta(\{i_1\}^C) = \mathbf{0} \\ \beta(i_1) \geq 0 }}  L(\beta),
% \end{align}

% \textbf{Following saddles.} We can recursively follow the previous logic to compute the jump times and the following saddles. However one must be careful in not forgetting the sign constraints. 

% Our saddle-to-saddle algorithm is formally outlined in \cref{alg:algo}. This procedure enables to identify and characterise the saddles as well as the jump times of the limiting dynamics. We first verify that all the steps are well defined and that the algorithm terminates in a finite number of iterations in the following proposition.  The proof is deferred to \Cref{app:sec:proofprop2}. \note{see if we add the prop or not}


% \normalsize

==> Sections/main_result_v2.tex <==
\section{Existence and construction of the limiting dynamics}\label{sec:main}
%



%COLT
% \RestyleAlgo{ruled}
% \begin{algorithm}[t] 
% \caption{Successive saddles and jump times of $\lim_{\alpha \to 0} \tilde{\beta}^\alpha$}\label{alg:algo}
% \KwData{$X \in \R^{n \times d}$, $y \in \R^n$}
% % \KwResult{$y = x^n$}
% \ \ $(t, \beta, s,r ) \gets (0, \mathbf{0}_d, \mathbf{0}_d, - \nabla L(\mathbf{0_d}))$ \; \\ 
% \While{$r \neq \mathbf{0}$}{
% % \ \ $A = \{i \in [d] \text{ s.t. } r(i) \neq 0\}$   \\
% \ \ $\Delta \gets \inf \big \{ \delta > 0  \text{ s.t. } \exists i \in \{j \in [d], r(j) \neq 0\} ,   s(i) + \delta r(i) = \pm 1  \big \}$ \\ 
% $s \gets s + \Delta \cdot r$ \\ 
% $t \gets t + \Delta$ \\
% $I_{\pm} \gets \{i \in  [d] \text{ s.t. }  s(i) = \pm 1 \} $ \\ 
% $\beta \gets \underset{ \substack{ \beta_i \geq 0 , i \in I_+ \\ \beta_i \leq 0, i \in I_- \\ \beta_i = 0, i \notin I_+ \cup I_- } }{\text{arg min}} L(\beta) $ \\  
% $r \gets - \nabla L(\beta)$ 
% }
% \textbf{Output:} Successive values of $\beta$ and $t$
% \end{algorithm}


% \begin{algorithm}
% \caption{An algorithm with caption}\label{alg:cap}
% \begin{algorithmic}
% \Require $n \geq 0$
% \Ensure $y = x^n$
% \State $y \gets 1$
% \State $X \gets x$
% \State $N \gets n$
% \While{$N \neq 0$}
% \If{$N$ is even}
%     \State $X \gets X \times X$
%     \State $N \gets \frac{N}{2}$  
% \ElsIf{$N$ is odd}
%     \State $y \gets y \times X$
%     \State $N \gets N - 1$
% \EndIf
% \EndWhile
% \end{algorithmic}
% \end{algorithm}



% and simple computations lead to  $\tilde{\phi}_\alpha(\beta) \to \Vert \beta \Vert_1$ as $\alpha \to 0$ and its gradients satisfy  $[\nabla \tilde{\phi}_{\alpha}(\beta)]_i \to \pm 1$ if $\beta_i \gtrless 0$ (see \Cref{app:lemma:behaviour_nablaphia} in \Cref{app:sec:technical}).
% %


blablabla

\begin{thm}[Piecewise   constant  limiting   process]\label{thm:convergence}
There exist a number of jumps $p \in \N$, vectors $(\beta_0, \dots, \beta_p)$ and jump times  $(t_0 = 0, t_1, \dots, t_{p})$ such that, on any compact subset of $\R_{\geq 0} \backslash \{ t_1, \dots, t_p \}$,  the accelerated iterates $(\tilde{\beta}^\alpha_t)_{t}$ defined in \Cref{eq:rescaled_iterates} uniformly converge   towards the piecewise constant process $(\Tilde{\beta}^\circ_t)_t$ defined as: 
\begin{align*}
\tilde{\beta}^\circ_t \equiv \beta_k \qquad \qquad \text{    for   }  t \in (t_{k}, t_{k+1}) \text{   and   } 0 \leq k \leq p,  \ \ t_{p+1} = + \infty.
\end{align*}
\end{thm}




The previous theorem provides the existence of a limiting dynamics. The goal is now to determine the values of the times  $(t_0 = 0, t_1, \dots, t_{p})$ as well as of the vectors $(\beta_0, \dots, \beta_p)$. To do so, it is natural to examine the limiting equation obtained when taking the limit $\alpha \to 0$ in \Cref{eq:process_integral_form}. We first turn it to its integral form which writes:
\begin{align}\label{eq:process_integral_form2}
      - \int_0^t \nabla L(\ttbeta_s^\alpha) \dd s =\nabla \ttphi_\al( \ttbeta_t^\al).
\end{align}
The uniform boundedness of the functions $\tilde{\beta}^\alpha$ (see ref in the appendix) along with the uniform convergence on compact subsets from \Cref{thm:convergence} gives that the left hand side of the previous equation converges to $- \int_0^t \nabla L(\ttbeta^\circ_s) \dd s$. For the right hand side, recall that $\ttphi_\alpha(\beta) \sim \Vert \beta \Vert_1$ as $\alpha \to 0$,  it is therefore natural to expect the right hand side of \Cref{eq:process_integral_form2} to converge towards an element of $\partial \Vert \ttbeta^\circ_t \Vert_1$, where we recall the definition of the subderivative of the $\ell_1$-norm as:
\begin{align*}
 \sg{\tilde{\beta}} = 
       \ \{1\} \ \  \text{if} \ \ \   \tilde{\beta} > 0, 
      \quad  \ \{-1\} \ \ \text{if} \ \   \tilde{\beta} < 0,
      \quad  \ [-1, 1] \ \  \text{if} \ \  \tilde{\beta} = 0 .
\end{align*}
% We start by providing a few comments concerning \Cref{eq:limit_process}.
The previous intuition can be shown to be correct and we defer the proof to the appendix (see REF). We can now write the key equation which must follow the limiting process.


\begin{prop}[Limiting equation]\label{prop:key_equation}
For all $t \geq 0$, the limiting process $\tilde{\beta}^\circ$ must satisfy:
\begin{align}\label{eq:key_equation}
    - \int_0^t \nabla L(\ttbeta^\circ_s) \dd s \in \partial \Vert \ttbeta^\circ_t \Vert_1.
\end{align}
\end{prop}

We show below that \Cref{eq:key_equation} uniquely determines the number of jumps $p$ as well as jump times and visited vectors, which turn out to be saddles. First, we point out the link between our limiting equation and the Lasso \citep{santosa1986linear,tibshirani1996regression}.





\myparagraph{Links with Lasso.}
Recall that the Lasso problem is formulated problem:
% Notice that \Cref{eq:key_process} closely resembles to the Lasso optimality condition: 
\begin{align}\label{eq:LASSO}
  \beta^\star_\lambda= \argmin_{\beta \in \R^d} \ L(\beta) + \lambda \Vert \beta \Vert_1.
\end{align}
The optimality condition of \Cref{eq:LASSO} writes $- \nabla L(\beta^\star_\lambda) \in \lambda \sg{\beta_\lambda^\star}$. Now notice the similarity with equation \Cref{eq:key_equation}: the two would be equivalent with $\lambda = 1 / t$ if the integration on the left hand of side of \Cref{eq:key_equation} did not average over the whole trajectory but only on the final iterate, in which case $- \int_0^t \nabla L(\ttbeta^\circ_t) \dd s = - t \cdot \nabla L(\ttbeta^\circ_t)$.  Though the difference is small, the trajectories of our limiting trajectory $\ttbeta^\circ$ and the lasso path $(\beta^\star_\lambda)_\lambda$ are quite different: indeed one has jumps, whereas the other is continuous. In fact, for the quadratic loss, the regularisation path $(\beta^\star_\lambda)_{\lambda \geq 0 }$ is a piecewise linear path with a discrete number of vertices. It can be computed using the  Homotopy algorithm~\citep[see, e.g.,][and references therein]{tibshirani2013lasso}. Starting from $\beta^\star_{\lambda \to \infty} = 0$ the overall idea behind the method is: \textit{\textbf{(i)}} compute the unique direction in which the iterates can evolve and move along it \textit{\textbf{(ii)}} find the value of $\lambda$ at which the optimality condition  $- \nabla L(\beta^\star_\lambda) \in \lambda \sg{\beta^\star_\lambda}$ breaks \textit{\textbf{(iii)}} update the direction accordingly and repeat. This procedure is iterated a finite number of times until reaching the minimum $\ell_1$-norm solution: $\beta^\star_{\lambda \to 0} =\beta^\star_{\ell_1}$.

Though our equation \Cref{eq:key_equation} is slightly different to that of the Lasso, it turns out that we can follow the same spirit behing the Homotopy algorithm to compute the jump times $(t_0, \dots, t_p)$ and saddles $(\beta_0, \dots, \beta_p)$.

% The algorithm we end up shares the same flavours as the Homotopy algorithm.

% to gradually construct the unique path which maintains the optimality condition $- \nabla L(\beta^\star_\lambda) \in \lambda \sg{\beta^\star_\lambda}$ satisfied by computing the vertices which correspond to values of $\lambda$ at which the optimality condition "is about to break".


% and $\beta^\star_{\lambda \to 0} =\beta^\star_{\ell_1}$. This re

% iteratively be computed starting from $\beta^\star_{\lambda \to \infty} = \mathbf{0}$ until reaching the minimum $\ell_1$-norm solution $\beta^\star_{\lambda \to 0} = \beta^\star_{\ell_1}$. \

% through the

% which operates in an iterative fashion and finds each vertex starting from $\mathbf{0}$. 
%





%\vspace*{0.2em}
% \subsection{Intuitive proof of \Cref{thm:main_theorem}}\hspace*{0.001em}

%\vspace*{0.5em}
% We provide here an intuitive sketch of the proof of \Cref{thm:main_theorem} assuming that the limiting process exists. Note that this \textbf{is not} a rigorous proof but has the advantage of preserving intuitive comprehension (the full proof is a consequence of \Cref{th:rescaled_time} and can be found \Cref{app:proof:thm2}).
%has the benefit of keeping things intuitive. 
% The idea is similar to the Homotopy algorithm which is used to find the Lasso path: we start from $\mathbf{0}$ and successively look at the breaking times of \Cref{eq:limit_process} and determine the unique update of $\tilde{\beta}_t$ that keeps the conditions satisfied.

\paragraph{Construction of the saddle-to-saddle algorithm.}
In the following, for a vector $v \in \R^d$ we denote by $v[i] \in \R$ its $i^{th}$ coordinate, we use the notation $v \in (-1, 1)$ to say that $v[i] \in (-1, 1)$, $\forall i \in [d]$. Let us denote $s_t \coloneqq - \int_0^t \nabla L(\tilde{\beta}^\circ_s) \dd s$.  This function has $4$ key properties which will be crucial for the construction of the limiting process:


\begin{enumerate}[leftmargin=15.2mm,label=(K\textbf{\arabic*}),ref=(K\arabic*)]
  \setcounter{enumi}{0}
\item
\label{prop1}
$t \mapsto s_t$ is continuous
\item
\label{prop2}
 For all $t \geq 0$, $s_t \in [-1, 1]$
\item 
\label{prop3}
For $i \in \R^d$, $s_t[i] \in (-1, 1) \Rightarrow \beta^\circ_t[i] = 0$
\item 
\label{prop4}
For $i \in \R^d$, $s_t[i] = 1 \Rightarrow \ttbeta^\circ_t[i] \geq 0$ and  $s_t[i] = -1 \Rightarrow \ttbeta^\circ_t[i] \leq 0$
\item 
\label{prop5}
For $i \in \R^d$, $\ttbeta^\circ_t[i] > 0 \Rightarrow  s_t[i] = 1$ and $\ttbeta^\circ_t[i] < 0 \Rightarrow  s_t[i] = -1$
\end{enumerate}

Items \ref{prop2} to  \ref{prop5}  are direct consequences of \Cref{prop:key_equation}. 

% The function $s_t$ is therefore continuous and, as noted in \Cref{eq:limit_process}, satisfies $s_t \in \partial \Vert \tilde{\beta}_t \Vert_1$.


\textbf{Original saddle: the iterates are stuck at $\mathbf{0}$.}  Intuitively one can think of the proof as a "continuous recursion" as follows: $\beta_t = \mathbf{0}$ on $[0, t)$ implies, by its definition, that $s_t = - t \cdot \nabla L(\beta_0)$. Now from \Cref{prop3}  $s_t \in (-1, 1)$ implies $\beta_t = \mathbf{0}$ . This "recursion" holds until a coordinate of $- t \cdot \nabla L(\beta_0)$ hits $\pm 1$. 
% Since $s_{t = 0} = \mathbf{0}$ and $s_t$ is continuous, there exists $\varepsilon > 0 $ such that $s_t \in (-1, 1)$ for $t \in [0, \varepsilon]$ and therefore $\ttbeta_t^\circ = \mathbf{0}$ (from 2). Hence $s_t = - t \cdot \nabla L(\beta_0 = \mathbf{0})$. 
For a rigorous proof, let $t_{\mathrm{break}} = \inf \{ t \geq 0, \exists i \in [d], s_t[i] = \pm 1 \} \in \R \cup \{+\infty\}$. Since $s_{t = 0} = \mathbf{0}$ and $s_t$ is continuous, we have that $t_{\mathrm{break}} > 0$ and that $s_t \in (-1, 1)$ for $t \in [0, t_{\mathrm{break}})$, from \ref{prop3} this means that $\beta_t = \mathbf{0}$ and therefore $s_t = - t \cdot \nabla L(\beta_0 = \mathbf{0})$ for $t \in [0, t_{\mathrm{break}})$. The definition of $t_{\mathrm{break}}$ can now be rewritten as $t_{\mathrm{break}} = \inf \{ t \geq 0, \exists i \in [d], -t \cdot \nabla L(\beta_0) = \pm 1 \} = 1 / \Vert \nabla L(\beta_0) \Vert_\infty $. Let $i_{\mathrm{break}}$ be the coordinate which reaches $\pm 1$ at time $t_{\mathrm{break}}$. For simplicity assume that it is unique, and w.l.o.g. assume that $s_t(i_{\mathrm{break}}) = +1$.

\textbf{The iterates must jump.} At time $t_{\mathrm{break}}$, we now show that: (i) the coordinate $i_{\mathrm{break}}$ must jump, (ii) the others must stay at $0$. Consider an interval $t \in (t_{\mathrm{break}}, t_{\mathrm{break}} + \varepsilon)$. Indeed by \ref{prop1}, $s_t(\{ i_{\mathrm{break}} \}^C ) \in (-1, 1)$, and hence $\ttbeta^\circ_t( \{ i_{\mathrm{break}} \}^C ) = \mathrm{0}$ from \ref{prop3}. Now assume that $\beta_t(i_{\mathrm{break}})$ is still equal to $0$ for $t \in (t_{\mathrm{break}}, t_{\mathrm{break}} + \varepsilon)$, then $s_t$ would still be equal to $-t \cdot \nabla L(\beta_0 = \mathbf{0})$ and $s_t(i_{\mathrm{break}}) > 1$ which contradicts contradicting \ref{prop2}. Therefore the first jump time is $t_{\mathrm{break}}$:   $t_1 = t_{\mathrm{break}}$.

\textbf{Saddle $\beta_1$?} The question is now to determine, where the iterates have jumped: i.e., what is the value of $\beta_1$ for $t \in (t_1, t_2)$? As shown in the previous paragraph: $\ttbeta^\circ_t(\{ i_{\mathrm{break}} \}^C) = \beta_1(\{ i_{\mathrm{break}} \}^C )= \mathbf{0}$ and $\beta_1( i_{\mathrm{break}}  ) \neq 0$. Recall that w.l.o.g we assumed that $s_{t_1}(i_{\mathrm{break}}) = +1$, therefore from \ref{prop4}, $\beta_1( i_{\mathrm{break}}  ) > 0$ and from \ref{prop5}, $s_t(i_{\mathrm{break}}) = 1$ for $t \in (t_1, t_2)$. On the other hand, from the definition of $s_t$ we can also write, $s_t(\ib) = +1 - (t-t_1) [\nabla L(\beta_1)]_\ib $ which leads to $[\nabla L(\beta_1)]_\ib = 0$. Notice that the two conditions $\beta_1(\{ i_{\mathrm{break}} \}^C )= \mathbf{0}$ and $[\nabla L(\beta_1)]_\ib = 0$ uniquely determines $\beta_1$ as being the unique solution of 
\begin{align}
    \beta_1 = \argmin_{\substack{\beta(\{i_1\}^C) = \mathbf{0} \\ \beta(i_1) \geq 0 }}  L(\beta),
\end{align}




% Now notice that $t_1$ defined in Algorithm \ref{alg:algo} corresponds to the time such that $\Vert s_{t_1}\Vert_{\infty}  = \pm 1$. The iterates must then move: indeed assume that $\tilde{\beta}_{t}$ is still $\mathbf{0}$ for $t \in [t_1, t_1 + \varepsilon]$, then we would have $\Vert s_t \Vert_\infty > 1$ which contradicts \Cref{eq:limit_process}. For simplicity, assume that there is a unique coordinate $i_1$ such that $|s_{t_1}(i_1)| = 1$ and without loss of generality assume that $s_{t_1}(i_1) = +1$.



% \textbf{Second saddle: $(t_1, t_2)$.} The iterates have jumped to another saddle point which we denote $\beta_1$, the question is now to determine which precise saddle it is. First note that by continuity of $s_t$ at time $t_1$ and because $\Vert s_{t_1}(\{i_1\}^C) \Vert_\infty < 1$ we must have $\beta_1(\{i_1\}^C) = \mathbf{0}$ from \Cref{eq:limit_process}. Furthermore, since we assumed that $s_{t_1}(i_1) = 1$, we must have that $\beta_1(i_1) \geq 0$. Therefore, we necessary have 
% \begin{align}
%     \beta_1 = \argmin_{\substack{\beta(\{i_1\}^C) = \mathbf{0} \\ \beta(i_1) \geq 0 }}  L(\beta),
% \end{align}
% which matches the first loop of Algorithm \ref{alg:algo}. Then $\ttbeta_t$ stays constant at $\beta_1 $ until time $t_2$ when an inactive coordinate $i_2$ is such that $s_{t_2}(i_2) = \pm 1$.
% % We have $I_0 = I_{0, \pm} = \emptyset$. 

\textbf{Following saddles.} We can recursively follow the previous logic to compute the jump times and the following saddles. However one must be careful in not forgetting the sign constraints. 

Add figure with illustrative example.

The following algorithm should now make complete sense.


\SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled}
\begin{algorithm}[h!]
\caption{Successive saddles and jump times of $\lim_{\alpha \to 0} \tilde{\beta}^\alpha$\label{alg:algo}}
\KwData{$X \in \R^{n \times d}$, $y \in \R^n$}
 $(t, \beta, s,r ) \gets (0, \mathbf{0}_d, \mathbf{0}_d, - \nabla L(\mathbf{0_d}))$ \; 
\While{$r \neq \mathbf{0}$}{
% % \ \ $A = \{i \in [d] \text{ s.t. } r(i) \neq 0\}$   \\
 $\Delta \gets \inf \big \{ \delta > 0  \text{ s.t. } \exists i \in \{j \in [d], r(j) \neq 0\} ,   s(i) + \delta r(i) = \pm 1  \big \}$ \\ 
$(t, \ s) \gets (t + \Delta, \ s + \Delta \cdot r) $ \\ 
$I_{\pm} \gets \{i \in  [d] \text{ s.t. }  s(i) = \pm 1 \} $ \\ \vspace{0.2em}
$\mathrm{Constraints} \gets \Big \{\beta \in \R^d \ \ \mathrm{s.t.}   \substack{ \beta_i \geq 0 \ \mathrm{if} \  i \in I_+ \\ \beta_i \leq 0 \ \mathrm{if} \  i \in I_- \\ \quad \ \ \beta_i = 0 \ \mathrm{if} \  i \notin I_+ \cup I_- } \Big \}  $ \\
\vspace{0.2em}
$\beta \gets \underset{\beta \in \mathrm{Constraints}  }{\text{arg min}} L(\beta) $  \\  
$r \gets - \nabla L(\beta)$ 
}
\textbf{Output:} Successive values of $\beta$ and $t$
\end{algorithm}

% Indeed a coordinate cannot jump from a strictly positive value to a strictly negative value since crossing $0$ always corresponds to a fixed point of the dynamics. This feature also appears in \Cref{eq:limit_process}: the function $s_t$, being continuous at the jump times, cannot pass from a value of $+1$ to $-1$ instantly.





% Our main result formalises the informal theorem given in the introduction.  The limiting flow progresses by jumping from one saddle to another, where each saddle corresponds to the minimiser of the loss function under constraints on the set of active coordinates and their sign.
% 
% that is restricted to a specific set of active coordinates. 
%




% We can now state our main result. We show that at vanishing initialisation, the limiting flow progresses by jumping between different saddles, where each saddle corresponds to a minimiser of the loss function subject to specific sign constraints. 






\begin{restatable}[Full description of the limiting process]{thm}{thmone}\label{thm:main_theorem}
Let the ``saddles'' $(\beta_0 = \mathbf{0}, \beta_1, \dots, \beta_{p-1}, \beta_p=\beta^\star_{\ell_1})$ and jump times $(t_0 = 0, t_1, \dots, t_{p})$ be the outputs of Algorithm \ref{alg:algo} and let  $(\Tilde{\beta}^\circ_t)_t$ be the piecewise constant process defined as follows:
\begin{align*}
 &\textbf{(``Saddles'')}   &&\tilde{\beta}^\circ_t \equiv \beta_k \qquad \qquad \text{    for   }  t \in (t_{k}, t_{k+1}) \text{   and   } 0 \leq k \leq p,  \ \ t_{p+1} = + \infty.
\end{align*}
The accelerated flow $(\tilde{\beta}^\alpha_t)_{t}$ defined in \Cref{eq:rescaled_iterates} uniformly converges towards the limiting process $(\Tilde{\beta}^\circ_t)_t$ on any compact subset of $\R_{\geq 0} \backslash \{ t_1, \dots, t_p \}$. 
\end{restatable}
% Let us comment our result.
\myparagraph{Behaviour of the saddle-to-saddle process.} The visited ``saddles''  are entirely provided in a recursive manner by Algorithm \ref{alg:algo}. 
Unlike all previous results on incremental learning, complex behaviours can occur when the feature matrix is ill designed and the RIP property~\citep{candestao} is not satisfied. Several coordinates can activate and deactivate at the same time (in \Cref{fig1} (Right), $4$ coordinates deactivate at the same time, in \Cref{app:fig} (Right), two coordinates activate at the same time). Moreover, there is no monotonicity of the total number of non-zero coordinates and each coordinate can increase, decrease and change sign many times. 


\myparagraph{Convergence result.} First we point out that we could not expect uniform convergence of $(\tilde{\beta}^\alpha_t)$ on intervals of the form $[0, T]$ given the fact that the limit process is discontinuous. Hence the uniform convergence outside of the discontinuity times is one of the strongest we could expect. In \Cref{cor:graph_convergence} in the following section we give an even stronger result by showing a graph convergence of the iterates. We also highlight that showing the convergence to a limiting process is in fact the toughest challenge from a theoretical point of view and is done \Cref{sec:rescaled}. However, in \Cref{subsec:construction}, assuming its existence, we show that constructing $\tilde{\beta}^\circ$ is rather intuitive and naturally leads to Algorithm \ref{alg:algo}.

\myparagraph{Estimate for the iterates $\beta^\alpha_t$.} We point out that our result provides no speed of convergence of $\tilde{\beta}^\alpha$ towards $\tilde{\beta}^\circ$. 
We believe that a non-asymptotic result is challenging and leave it as future work.
We experimentally notice that the convergence rate quickly degrades after each saddle. Nonetheless,  we can still write for the ``non-accelerated'' iterates that $\beta^\alpha_t = \tilde{\beta}^\alpha_{t / \ln(1 / \alpha)} \sim \tilde{\beta}^\circ_{t / \ln(1 / \alpha)} $ when $\alpha \to 0$. This approximation tells us for $\alpha$ small enough that the iterates $\beta^\alpha_t$ are roughly equal to $0$ until time $t_1 \cdot \ln(1/\alpha)$ and that  the minimum $\ell_1$-norm interpolator is reached at time $t_p \cdot \ln(1 / \alpha)$. Such a precise estimate of the global convergence time is  remarkable and goes beyond classical Lyapunov analysises which only leads to $L(\beta^\alpha_t) \lesssim \ln(1/\alpha) / t$ (see \Cref{app:prop:convergence_rates} in \Cref{app:sec:mirrorflow}).

\myparagraph{``Neural''  point of view.} We can map back our result to the accelerated flow $\tilde{w}^\alpha_t \coloneqq w^\alpha_{\tilde{t}^\alpha(t)}$. Indeed there is a bijective mapping between the mirror flow $\tilde{\beta}^\alpha_t$ and the gradient flow as shown in \Cref{app:lemma:bijection} in the appendix. 
From there we can show that 
$(\tilde{u}^\alpha_t, \tilde{v}^\alpha_t) \ \underset{\alpha \to 0}{\longrightarrow} \ (\sqrt{\vert \tilde{\beta}^\circ_t \vert}, \mathrm{sign}( \tilde{\beta}^\circ_t ) \sqrt{ \vert \tilde{\beta}^\circ_t \vert }  )$ uniformly on any compact subset of $\R_{\geq 0} \backslash \{ t_1, \dots, t_p \}$.
 %It is clear that the points $(\beta_k)_{k \in [p]}$ 
Also, we emphasise that the $\beta_k$'s which we refer to as ``saddles'' \textbf{are not} saddles of the convex loss $L$. We use this terminology as the mapping $(u_k,\!v_k) \!=\! (\sqrt{\vert \beta_k \vert}, \mathrm{sign}(\beta_k) \sqrt{\vert \beta_k \vert} )$ results in actual saddle points of the non-convex function~$F$.

\paragraph{Comment concerning the general position assumption \Cref{ass:general_pos}} This assumption is common in the Lasso framework as it ensures that the Lasso solution is unique for any regularisation parameter, in our case it similarly ensures that the constrained minimisation problem in saddle-to-saddle algorithm has a unique minimum as shown \Cref{lemma:alg_defined}.  Also, in the overparametrised setting, this assumption ensures that the minimum $\ell_1$-norm interpolator is unique~\citep[Theorem 2.2]{MR2887848}, we can therefore define $\beta^\star_{\ell_1} \coloneqq \argmin_{y_i = \langle x_i, \beta^\star \rangle, \forall i} \Vert \beta^\star \Vert_1$. 
Note that this assumption is not restrictive as it holds almost surely when the data is drawn from a continuous probability distribution~\citep[Lemma 4]{tibshirani2013lasso}. \color{black}









%\vspace*{0.5em}
% \subsection{Intuitive construction of the limiting process\label{subsec:construction}}\hspace*{0.001em}

%\vspace*{0.2em}




%\vspace*{0.3em}
\subsection{Additional comments} 
\hspace*{0.01em}
% \vspace*{0.2em}
%

\myparagraph{Comparisons to the Homotopy and OMP algorithms.} 
The jump times as well as the visited saddles depend on all the previously visited saddles, and not just on the last one. This behaviour is in stark contrast with the Homotopy algorithm for the Lasso. 
On a separate note, a common belief is that in the vicinity of a saddle point, the following activated coordinate should correspond to the direction of most negative curvature (i.e. eigenvector corresponding to the most negative eigenvalue). However, this statement cannot be accurate as it is inconsistent with our algorithm (though it holds true for the first coordinate).
%However this cannot be true as it is does not match our algorithm (it however holds for the first coordinate). 
%
In fact, it can be shown that by selecting this particular active coordinate
the resulting algorithm aligns with the orthogonal matching pursuit (OMP) algorithm~\citep{pati1993orthogonal,davis1997adaptive} which does not necessarily lead to the minimum $\ell_1$-norm interpolator.


\myparagraph{Natural extensions of our setting.} More general initialisations than $u_{t=0} = \sqrt{2} \alpha \mathbf{1}$ can easily be dealt with. For instance, initialisations of the form $u_{t=0} = \alpha \mathbf{u_0} \in \R^d$ lead to the exact same result as it is shown in~\cite{woodworth2020kernel} (Discussion after Theorem 1) that the associated mirror still converges to the $\ell_1$-norm. Initialisations of the form $[u_{t = 0}]_i = \alpha^{k_i}$, where $k_i > 0$, lead to the associated potential converging towards a weighted $\ell_1$-norm and one should modify Algorithm \ref{alg:algo} by accordingly weighting $\nabla L(\beta)$ in the algorithm. Similarly, deeper linear architectures of the form $\beta_w = w_+^D - w_-^D$ as in \cite{woodworth2020kernel} do not change our result as the associated mirror converges towards the $\ell_1$-norm too. Only the square loss is considered in the paper, however we believe that all our results should hold for any loss of the type $L(\beta) = \sum_{i=1}^n \ell(y_i, \langle x_i, \beta \rangle)$ where for all $y \in \R$,  $\ell(y, \cdot)$ is strictly convex with a unique minimiser at $y$. In fact, the only property which cannot directly be adapted from our results is showing the uniform boundedness of the iterates (see discussion before \Cref{app:prop:bounded_iterates} in \Cref{app:sec:mirrorflow}). 


